Multi-directional Geodesic Neural Networks via Equivariant Convolution

We propose a novel approach for performing convolution of signals on curved surfaces and show its utility in a variety of geometric deep learning applications. Key to our construction is the notion of directional functions defined on the surface, which extend the classic real-valued signals and which can be naturally convolved with with real-valued template functions. As a result, rather than trying to fix a canonical orientation or only keeping the maximal response across all alignments of a 2D template at every point of the surface, as done in previous works, we show how information across all rotations can be kept across different layers of the neural network. Our construction, which we call multi-directional geodesic convolution, or directional convolution for short, allows, in particular, to propagate and relate directional information across layers and thus different regions on the shape. We first define directional convolution in the continuous setting, prove its key properties and then show how it can be implemented in practice, for shapes represented as triangle meshes. We evaluate directional convolution in a wide variety of learning scenarios ranging from classification of signals on surfaces, to shape segmentation and shape matching, where we show a significant improvement over several baselines.

==> review.tex <==
\begin{Definition}[Levi-Civita connection]
Let $M$ be a Riemannian manifold and $g^M$ the metric of $M$. An affine connection on $M$ is a bilinear map:
\[
\begin{array}{rcl}
\nabla :\Gamma(TM, X) \times \Gamma(TM, M) & \rightarrow & \Gamma(TM, M)\\
(X, Y) &\mapsto & \triangledown_X Y
\end{array}
\]
such that for any smooth function $f: M \rightarrow \RR$ and vector fields $(X, Y) \in \Gamma(TM, M)^2$ we have:
\begin{itemize}
\item $\triangledown_{fX} Y = f.\nabla_{X} Y$
\item $\triangledown_{X} f.Y = (X.f).Y + f.\nabla_{X} Y$ (Leibniz rule)
\end{itemize}
There an unique affine connexion on $M$ called Levi-Civita connection satisfying the following conditions:
$\forall X, Y, Z \in \Gamma( TX, M)$, 
\begin{itemize}
\item $X.g^M( Y, Z ) = g^M( \nabla^M_X Y, Z) + g^M( \nabla^M_X Y, Z)$ \\
(metric compatibility)
\item $(\nabla^M_X Y - \nabla^M_Y X).f = X.f-Y.f$ (torsion free).
\end{itemize}
We denote by $\nabla^M$ the Levi-Civita connection of $M$.
\end{Definition}

\begin{Definition}[Pull-back connection]
Let $\nabla$ be a connection on a Riemannian manifold $N$ and $\varphi: M \rightarrow N$ a map between Riemannian manifolds. There is a pull-back connection:
\[
\varphi^{*}\nabla: \Gamma(TM, M) \times \Gamma(\varphi^*TN, M)  \rightarrow  \Gamma(\varphi^*TN, M)
\]
uniquely determined by the condition:
\[
(\varphi ^{*}\nabla )_{X}(\varphi ^{*}s)=\varphi ^{*}(\nabla _{\mathrm {T} \varphi (X)}s).
\]
\end{Definition}

\begin{Definition}[Parallel transport]
Let $X$ be a Riemannian surface and $\gamma : [0, 1] \rightarrow X$ a smooth immersion and let $s_0 \in \gamma^*TX$. There exists a unique section $s \in \Gamma(\gamma^*TX, [0, 1])$ such that:
\begin{itemize}
\item $s(0) = s_0$
\item $\gamma^*\nabla^X_{\scalebox{0.65}{$\frac{d}{dt}$}} s = 0$
\end{itemize}
This induces linear isometry:
\[
\rho_{\gamma}^X : T_{\gamma(0)} X = \gamma^*TX_0 \longrightarrow  T_{\gamma(1)} X = \gamma^*TX_1
\]
defined by $\rho_{\gamma}^X(s_0) = s(1)$ called parallel transport of $X$ along the path $\gamma$.
\end{Definition}

\begin{Definition}[Orthonormal frame bundle]
The orthonormal frame bundle of a Riemannian manifold $X$ is the fiber bundle $F_{\mathrm{O}}X$ whose fiber over $x \in X$ is the set of orthonormal bases of $T_x X$ for the inner product $g_x^X$ induced by the metric $g^X$.
\end{Definition}


\begin{Definition}[exponential map]
Let $X$ be a Riemannian manifold. The exponential map of $X$ is the map
\[
\begin{array}{l|rcl}
\exp^X : & TX & \longrightarrow & X \\
    & v \in T_x X & \longmapsto & \exp^X_x( v ) 
\end{array}
\]
where $\exp^X_x( v )$ is the point at time $1$ of the geodesic starting at $x$ with tangent vector $v$.
\end{Definition}

The exponential map of $X$ induces a family of maps $\exp^X_x: T_x X \rightarrow X$. Let $x \in X$ we can pull-back the metric of $X$ to $T_x X$ by $\exp^X_x$, this makes $T_x X$ into a Riemannian manifold. Denote by $\mu_x^X$ the associated measure. Let $x \in X$, a couple $e = (\lambda, u) \in \RR_+^* \times (F_{\mathrm{O}} X)_x$ induces a linear map from $T_x X$ to $\RR^n$ by sending each vector $\lambda.u_i$ to the $i$-th vector of the canonical basis of $\RR^n$ therefore for any function $f: T_x X \rightarrow Y$ we can consider its pull-back by $e^{-1}$, $(e^{-1})^*f : \RR^n \rightarrow Y$. 

\begin{Definition}[Frame transporter]
Let $X$ be a Riemannian manifold and $x \in X$. For any $v \in T_x X$ denote by:
\[
\begin{array}{l|rcl}
\gamma_x^v : & [0,1] & \longrightarrow & X \\
    & t & \longmapsto & \exp_x^X(t.v)
\end{array}
\]
the associated parallel transport $\rho_{\gamma_x^v}^X: T_x X \rightarrow T_{\exp_x^X(v)} X$ being an isometry it induces a map 
\[
F^X_x(v,\bullet) : (F_{\mathcal{O}} X)_x \rightarrow (F_{\mathcal{O}} X)_{\gamma_x^v(1)}.
\]
We call the map:
\[
\begin{array}{l|rcl}
F^X : & TX \times_X F_{\mathrm{O}}X & \longrightarrow & F_{\mathrm{O}}X \\
    & (v,e) \in T_x X \times (F_{\mathrm{O}} X)_x & \longmapsto & F^X_x(v,e) \end{array}
\]
the frame transporter of $X$.
\end{Definition}

==> trash.tex <==

\subsection{Synchronized Convolution in practice}

The expression $(3)$ is coordinate free, however to implement it we must choose a representation of the data.
We represent tangent vectors in polar coordinates in their tangent plane. This representation implies an arbitrary choice of origin direction $e_x \in T_x X$ in each tangent plane. For any (non null ) tangent vector $v \in T_x X$ we denote by $e_x ( v )$ the angle corresponding to the vector $v$. We express directional functions as functions over $X \times [0, 2\pi[$ we call them angular functions. Given a directional function $\varphi$ we obtain an angular function $\varphi_e$ defined by:
\[
\varphi_e ( x, \theta ) := \varphi(x, e_x^{-1}( \theta )).
\]
We express the exponential map and the parallel transport with respect to $e_x$ for any radius $r > 0$ and angles $\theta, \theta_1, \theta_2 \in [0, 2\pi[:$
\[
\exp_{x, e_x}^X(r, \theta) := \exp_x^X( re_x^{-1}(\theta) )
\]
\[
\Gamma_{x, (r, \theta_1)}^{e}( \theta_2 ) := e_{\exp^X_{x, e_x}(r,\theta_1)} \big( \Gamma_{x, e_x^{-1}(\theta_1)} \big)
\]
\[
\overline{\exp}_{x}^{X,e}(r, \theta) = (\exp_{x, e_x}^X(r, \theta), \Gamma_{x, (r, \theta)}^{e}( \theta ))
\]
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.65]{images/transport_practice}
    \caption{Pull-back of angular function}
\end{figure}
we also express the kernel alignment map by:
\[
\tau_{x, \theta}^e := \tau_{x, e_x^{-1}(\theta)}.
\]
Given an angular function $\tilde{\varphi}$ we denote by $\tilde{\varphi} *_e k$ it synchronized convolution with kernel $k$:
\begin{align}
\tilde{\varphi} \star_e k (x,\theta) = \langle (\overline{\exp}^{X,e}_{x})^{*}\tilde{\varphi}, (\tau_{x,\theta}^e)^*k \rangle.
\end{align}
The following proposition/theorem shows that this construction of synchronized convolution is equivariant with respect to the choice of reference direction. Namely,
\begin{Proposition}
Let $e_x \in T_x X$ be a family of unit tangent vectors defined at every point $x \in X$ then for any family of rotation matrices $R_x$ of angle $\theta_x$ we have:
\[
\varphi_{R.e} \star_{R.e} k( x, \theta ) = \varphi_{e} \star_e k(x, \theta + \theta_x )
\]
Where $(R.e)_x := R_x.e_x$.
\end{Proposition}
\begin{proof}
\[
\varphi_{R.e}(x, \theta) = \varphi_{e}(x, \theta + \theta_x)
\]
\[
\tau_{x, \theta}^{R.e} = \tau_{x,\theta + \theta_x}^e.
\]
\[
\exp_{x, R.e_x}^X(r, \theta) = \exp_{x, e_x}^X(r, \theta + \theta_x)
\]
Thanks to orthogonality of parallel transport we have:
\[
\begin{aligned}
&
\Gamma_{x, (r, \theta_1)}^{R.e}( \theta_2 )
\\
&
= 
\Gamma_{x, (r, \theta_1+\theta_x)}^{e}( \theta_2 + \theta_x) + \theta_{\exp^X_{x, e_x}(r, \theta + \theta_x)}
\\
&
=
\Gamma_{x, (r, \theta_1+\theta_x)}^{e}( \theta_2 ) + \theta_x + \theta_{\exp^X_{x, e_x}(r, \theta + \theta_x)}
\end{aligned}
\]
Thus
\[
\begin{aligned}
&
(\overline{\exp}^{X,R.e}_{x})^{*}\varphi_{R.e}(x, (r,\theta)) 
\\
&
=
\varphi_{R.e}(\exp_{x, e_x}^X(r, \theta + \theta_x), \Gamma_{x, (r, \theta_1+\theta_x)}^{e}( \theta_2 ) + \theta_x + \theta_{\exp^X_{x, e_x}(r, \theta + \theta_x)}
\\
&
=
\varphi_e(\exp_{x, R.e_x}^X(r, \theta + \theta_x), \Gamma_{x, (r, \theta_1+\theta_x)}^{e}( \theta_2 ) + \theta_x)
\\
&
=:
(\overline{\exp}^{X,e}_{x})^{*}\varphi_{e}(x, (r,\theta + \theta_x)). 
\end{aligned}
\]
Hence:
\[
\begin{aligned}
&
\varphi_{R.e} \star_{R.e} k (x,\theta)
\\
&
= 
\langle (\overline{\exp}^{X, R.e}_{x})^{*}\varphi_{R.e}, (\tau_{x,\theta}^{R.e})^*k \rangle.
\\
&
=
\langle (\overline{\exp}^{X, e}_{x})^{*}\varphi_{e}(\bullet, \bullet + \theta_x), (\tau_{x,\theta+\theta_x}^e)^*k \rangle
\\
&
=
\varphi_{e} \star_{e} k (x,\theta + \theta_x)
\end{aligned}
\]
\end{proof}


To define an analogue of convolutional neural networks as defined in the previous section over triangle meshes we must discretize its key ingredients:
\begin{itemize}
\item Volume measure
\item Tangent space
\item Exponential map
\item Frame transporter
\end{itemize}

\begin{Definition}[Triangle mesh]
A triangle mesh $M$ is the data of two matrices $V^M \in M_{\mathrm{nv}(M), 3}$ and $F^M \in M_{\mathrm{nf}(M),3}(\mathbb{N})$. Such that for all $ i, j, F^M_{ij} \in [|1; \mathrm{nv}(M)|]$ and $F^M_{i,1}, F^M_{i,2}, F^M_{i,3}$ are distinct. The rows of $V^M$ are the vertices coordinates in $\RR^3$ and the rows of $F^M$ the triangles. We also require that two triangles have either $0$ or $2$ vertices in common and three triangles can’t have more than one vertex in common.
\end{Definition}

We refer to the vertices by the index of the corresponding row of $V^M$. Two vertices $ i,j$ are said to be neighbors if there exist a triangle containing them both, we denote this relation by $i \sim_M j$.
We say that a triangle $F_j$ is adjacent to a vertex $i$ if it contains $i$ and we also denote this relation by $F_j \sim_M i$. For any vertex $i$ we denote by:
\[
\mathcal{N}^M( i ) := \{ j \vert \ i \sim_M j, j \neq i\}
\]
its set of neighbors. We denote by $n^M(i) := |\mathcal{N}^M(i)|$ the number of neighbors of $i$.
\begin{Definition}[Volume measure]
The volume measure of a triangle mesh $M$ is the measure $\mu^M$ on the set of vertices of $M$ such that for each vertex $i$, $\mu^M_i$ is the sum of the areas of the triangles adjacent to $i$. 
\end{Definition}


\begin{Definition}[Neighbors listing procedure]
Let $i$ a vertex of a triangle mesh $M$ denote by:
\[
\mathcal{S}^M(i) := \{(j,k) \in \mathcal{N}^M(i)^2 \ \vert \ k \sim_M j \}
\]
Let $(s_1, s_2) \in \mathcal{S}^M(i)$, we define its successor $s_3 = s^M(j_1, j_2) \in \mathbb{N}$ to be the neighbor by the conditions $s_3 \neq j_2$, $s_3 \sim_M i$, $s_3 \sim_M s_2$ if they can be satisfied or by $-1$ otherwise. We can define the list $s = L^M(j_1, j_2)$ recursively by $s_{i+1} = s^M(s_{i-1},s_{i})$ until $s_i$ has already been listed or $s_i = -1$.
Denote by $l = l^M(s_1, s_2)$ the length of this list. If $l = n^M(i)$ for any choice of $(s_1, s_2)$ we say that $i$ is an interior point, otherwise we say that $i$ is a boundary point.
\end{Definition}
For simplicity we may assume that our mesh has no boundary points.
\begin{Definition}[Tangent bundle of a mesh]
Let $i$ be an interior vertex of a mesh $M$ let $s_1, \dots , s_{n^M(i)}$ a listing of $\mathcal{N}^M(i)$ according to the previously described procedure. For each $j$ denote by $e_j$ the edge $(i, s_{j})$ and by $\theta_j$ the angle between edges $e_j$ and $e_{(j+1) \  \mathbf{mod} \ n^M(i)}$ we normalize the $(\theta_j)$ to produce angles 
$
\alpha_j := (2\pi\theta_j)/(\sum_{k=1}^{n^M(i)} \theta_k)
$.
This gives polar coordinates on $D^M(i) := \{i\} \cup \mathcal{N}^M(i)$, $i$ being at the origin and $s_{j}$ having norm $\Vert V^M_{s_{j},\bullet} - V^M_{i,\bullet} \Vert_2$ and angle $\sum_{k = 1}^{i-1} \alpha_k$. Using this system of polar coordinates we an embedding $\iota: D^M(i) \hookrightarrow \RR^2$ and a surjective linear map $f: \mathrm{Span}_{\RR}((e_j)_j) \rightarrow \RR^2$ defined by $f(e_j) := 
\iota(s_j) - \iota(i)$ we define the tangent space $T_i M$ to $M$ at vertex $i$ to be the quotient space:
\[
T_i M = \mathrm{Span}_{\RR}(e_1, \dots, e_{n^M(i)}) \big/ \mathrm{Ker}(f) \simeq \RR^2. 
\]
This construction is independent of the particular choice of indexing made to construct the listing. The space $T_i M$ inherits the inner product of $\RR^2$. We denote by $g_i^M$ the inner product on $T_i M$ defined by: 
\[
g_i^M( e_j, e_{(j+1) \ \mathbf{mod} \ n^M(i)} ) = \alpha_i.\Vert e_j \Vert_2.\Vert e_{(j+1) \ \mathbf{mod} \ n^M(i)} \Vert_2.
\]
We denote by $\Vert \bullet \Vert_i^M$ the associated norm. The collection of tangent spaces $(T_i M)$ gives a bundle $TM$ over the discrete space of vertices of $M$ called the tangent bundle of $M$. Each tangent space being equipped with an inner product we also have a notion of orthonormal frame bundle $F_{\mathrm{O}} M$. 
\end{Definition}
Now that we have defined the tangent bundle we must define the exponential map and the frame transporter. The set of vertices of the mesh $M$ is discrete and the tangent space to a vertex being continuous it is more convenient to compute geodesic polar coordinates (GPC) (inverse of the exponential map) which gives us an embedding of the set of vertices to the tangent space. A construction of GPC inspired by the methods of fast marching \cite{sethian1999level} has been proposed in \cite{melvaer2012geodesic}. The idea is to compute GPC on $D^M(s)$ and to extend them to the whole mesh using an update procedure that takes the GPC estimates over two adjacent vertices and produces an estimate of the GPC over their common neighbors. We propose an extension of the update scheme to compute the frame transporter jointly. First we describe the update procedure at a vertex $i$ of $M$. For all vertex $i$ we denote by $r_{si}, \theta_{si}$ the estimates at $i$ of the radius and angle of the GPC centered at $s$. We list all $\mathcal{N}^M(i)$ according to the neighbors listing procedure. This defines GPC $(r_{ij}, \theta_{ij})$ on each $D^M(i)$ those GPC are defined up to cyclic permutation and order reversion of the listing. We can represent tangent vectors using these local GPC, in particular tangent vectors can be represented only by their angle. We denote by $u^1_{s}$ and $u^2_{s}$ the angles corresponding to the first and second vector of the orthonormal basis induced by the local GPC at vertex $s$ and by $u^1_{si}$ and $u^2_{si}$ the angles corresponding to the estimates of transport to vertex $i$. This gives us an estimate of the parallel transport along a "virtual" geodesic going from $s$ to $i$ in the bases $(u_s^1, u_s^2)$ and $(u_i^1, u_i^2)$. For all $(j,k) \in \mathcal{S}^M(i)$ denote by $e_{ij}, e_{ik} \in T_i M$ the corresponding edges considered as tangent vectors. Denote by $s_{ijk} \in T_i M$ the vector such that:
\[
\Vert e_{ij} - s_{ijk} \Vert_i^M = r_{sj}, \ \ \Vert e_{ik} - s_{ijk} \Vert_i^M = r_{sk}.
\]
The new estimate $\tilde{r}_{si}$ of the radius at $i$ is obtained by:
\[
\tilde{r}_{si,jk} := \min \big\{ \Vert y - s_{ijk} \Vert_i^M + \Vert y \Vert_i^M \ \big\vert \ y \in [e_{ij}, e_{ik}] \big\}.
\]
Denote by $y_{ijk} \in T_i M$ the vector achieving the above minimum, by $\phi_{ij}$ the angle between $e_{ij} - s_{ijk}$ and $-s_{ijk}$ and by $\phi_{kj}$ the angle between $e_{ij} - s_{ijk}$ and $e_{ik} - s_{ijk}$ and by $\alpha = \phi_{ij} / \phi_{ik}$. angles $a_1$ and $a_2$ they define two angular sectors, we suppose that one is smaller, thus it the one that smaller than $\pi$. For $t \in [0, 1]$ the convex combination $(1-t).a_1 + t.a_2$ can be defined in two ways depending on which angular sector we consider. We denote by $\mathrm{mix}(t, a_1, a_2)$ the angle corresponding to the convex combination according to the smaller angular sector. The update $\tilde{\theta}_{si}$ of the angle coordinate at vertex $i$ is defined by:
\[
\tilde{\theta}_{si,jk} 
:= 
\left\{
\begin{array}{l}
  \theta_{sj}, \ \text{if} \ \ y_{ijk} = e_{ij} \\
  \theta_{sk}, \ \text{if} \ \ y_{ijk} = e_{ik} \\
  \mathrm{mix}(\alpha, \theta_{ij}, \theta_{ik}), \ \text{else}
\end{array}
\right.
\]
We extend the update scheme to compute the parallel transport. We need a way to transfer unit vectors from a vertex $j$ to an adjacent vertex $i \sim_M j$. We have listings $s_{k,1}, \dots , s_{k,n^M(k)}$ of $\mathcal{N}^M(k)$ for all vertex $k$, define $i_{ji}$ by $i = s_{j,i_{ji}}$ we say that vertices $j$ and $i$ have compatible orientation if:
\[
s_{j,(i_{ji}+1) \ \mathbf{mod} \  n^M(j)} = s_{i,(i_{ij}-1) \ \mathbf{mod} \  n^M(i)}.
\]
If two vertices are not orientation compatible we can reverse the order of the listing of the second vertex to make them compatible. Starting from one seed vertex we can propagate its orientation to other vertices using a Dijkstra like traversal of the mesh, therefore we can assume that all adjacent vertices are orientation compatible. Let $u \in T_j M$ a unit tangent vector at $j$ given as an angle in the local GPC of $j$ then we define its transport along $e_{ji}$ by: 
\[
\rho_{ji}(u) = u + \theta_{ij} - \theta_{ji} + \pi. 
\]
The updates $\tilde{u}^{l}_{si}$ (for $l = 1, 2$) of the transported basis $(u^1_s, u^2_s)$ is defined by:
\[
\tilde{u}^{l}_{si,jk} 
:= 
\left\{
\begin{array}{l}
  \rho_{ji}(u^l_{sj}), \ \text{if} \ \ y_{ijk} = e_{ij} \\
  \rho_{ki}(u^l_{sk}), \ \text{if} \ \ y_{ijk} = e_{ik} \\
  \mathrm{mix}(\alpha, u^l_{ij}, u^l_{ik}), \ \text{else}
\end{array}
\right.
\]
For any vertex $i$ we denote by:
\begin{itemize}
\item $\tilde{r}_{si} := \min \big\{ \tilde{r}_{si, jk} \ \big\vert \ (j,k) \in \mathcal{S}^M(i) \big\}$.
\item $\tilde{\theta}_{si} := \tilde{\theta}_{si,jk}$ for $\tilde{r}_{si,jk} = \tilde{r}_{si}$.
\item $\tilde{u}_{si} := \tilde{u}_{si,jk}$ for $\tilde{r}_{si,jk} = \tilde{r}_{si}$.
\end{itemize}
We initialize the frame transport at each neighborhoods $D^M(i)$ by setting $u_{ii}^l = u^l_i$ and for all $j \in \mathcal{N}^M(i)$, $u^l_{ij} = \rho_{ij}(u^l_i)$. The basic structure of the algorithm for computing the GPC and frame transport centered at a vertex $s$ is the following:
\begin{algorithm}
\caption{GPC and frame transport algorithm}\label{}
\begin{algorithmic}[1]
\State $\mathrm{candidates.Empty}()$\Comment{free candidates list}
\For{$i = 1, \dots \mathrm{nv}(M)$}
\State $r_{si} = +\infty$
\EndFor
\State $\mathrm{initNeigbourhood}(s)$\Comment{init estimates on $D^M(s)$}
\State $\mathrm{candidates.Push}(D^M(s))$\Comment{add $D^M(s)$ to candidates}
\While{$\mathrm{candidates.notEmpty()}$}
\State $j = \mathrm{candidates.smallestNode()}$ \Comment{w.r.t. r}
\For{$k \in \mathcal{N}^M(j)$}
\If{$r_{si} > (1+\epsilon).\tilde{r}_{si}$} \Comment{precision $\epsilon > 0$}
\State \Comment{update estimates}
\State $r_{si} \gets \tilde{r}_{si}$
\State $\theta_{si} \gets \tilde{\theta}_{si}$
\State $u_{si} \gets \tilde{u}_{si}$
\State \Comment{if stopping criterion is not met}
\If{!$\mathrm{stopCriterion}(i)$}
\State \Comment{add $i$ to candidates}
\State $\mathrm{candidates.push(i)}$ 
\EndIf
\EndIf 
\EndFor
\EndWhile\label{endwhile}
\end{algorithmic}
\end{algorithm}

Different choices of stopping criterion are possible we may choose $\tilde{r}_{si} > R_{\mathrm{max}}$ to save computations and memory.






















\subsection{Patch operator}

\begin{Definition}[Patch operator]
Let $k : (\RR^n)^2 \rightarrow \RR$ a kernel for any $x \in X$ and $e \in F_x X$ we can pull it back to $\RR^n \times T_x X$ by $\mathrm{Id} \times e$. The (normalized) patch operator at $x$ associated to the kernel $k$ is the operator sending each function $f: X \rightarrow \RR$ to the function:
\[
\begin{array}{l|rcl}
f * k : & (X\times \RR^n) \times_X FX  & \longrightarrow & \RR \\
    & (y, e) \in \RR^n \times F_x X & \longmapsto & \frac{f * k(y, \bullet)(e)}{ 1 * k(y, \bullet)(e) } .
\end{array}
\]
where $(X\times \RR^n) \times_X FX = \bigsqcup_{x \in X} \RR^n \times F_x X$.
\end{Definition}
A close construction of the patch operator for surfaces has been proposed by Kokkinos et al.\cite{kokkinos2012intrinsic}.
In practice for surfaces it is more convenient to work with geodesic polar coordinates instead of exponential maps. That is around each point $x \in X$ we have an open subset $x \in U_x \subset X$ given a frame $e\in F_x X$ we have polar coordinates:
\[
\theta_x^e: U_x \rightarrow [0, 2\pi[, \ \ r_x^e: U_x \rightarrow \RR_+ 
\]
defined by:
\[
\left\{
\begin{array}{l}
  \theta_x^e(\exp_x^X(r(\cos(\theta)e_1 + \sin(\theta)e_2))
  =
  \theta
  \\
  r_x^e(\exp_x^X(r(\cos(\theta)e_1 + \sin(\theta)e_2))
  =
  r
\end{array}
\right.
\]
Following the construction of \cite{kokkinos2012intrinsic} we can define the patch operator at $x$ by:
\[
f * k (y, e)
:=
\frac{1}{K}\int_{U_x} f( z ) k(y, r_x^e(z) \exp(i \theta_x^e(z) ) ) d\mu^X( z )
\]
where 
\[
K 
=
K(x,y,e)
:=
\int_{U_x} k(y, r_x^e(z) \exp(i \theta_x^e(z) ) ) d\mu^X( z ).
\]
Note that if $k(y, r_x^e(\bullet) \exp(i \theta_x^e(\bullet) ) )$ is supported on $U_x$ for all $x \in X$ and $y \in \RR^n$ this construction coincides with our definition of patch operator. From now on we assume that we have a kernel $K$ is of the form:
\[
\begin{array}{l|rcl}
K : & (\RR^2)  & \longrightarrow & \RR_+ \\
    & (r_1e^{i\theta_1}, r_2e^{i\theta_2}) & \longmapsto & \tilde{K}(r_1, r_2, \theta_2 - \theta_1) .
\end{array} (*)
\]
for some map $\tilde{K}: \RR_+^2 \times S^1 \rightarrow \RR_+$ so that applying rotation on $\RR^2$ or on the tangent plane is equivalent in the sense that for any angle $\theta$ we have:
\[
f * K (e^{-i\theta}y, e) = f * K (y, \theta.e)
\]
where $\theta.e$ is the rotation of the frame $e$ by angle $\theta$. 

\subsection{Geodeisc convolutional neural networks}

In \cite{MasBosBroVan15} Boscaini et al. use the above patch operator construction to  introduce the notion of geodesic convolutional layer on which they build a deep learning framework. Suppose $X$ is an oriented surface the geodesic convolutional operator is defined for an arbitrary choice positively oriented frame $e_x$ at every point $x$ by:
\[
\mathrm{gc}(a, f)(x, \theta) 
:=
\int_{\RR_+} \int_{S^1} a(t - \theta, r)f*k(re^{it}, e_x) \ dt dr.
\]
for any weight function $a: S^1 \times \RR_+ \rightarrow \RR$. In a geodesic convolutional layer the map $a$ is discretized, the goal is to learn a vector contaning its values at certain locations. In general there is no canonical choice for the family $(e_x)_x$ therefore \cite{MasBosBroVan15} propose to follow the geodesic convolutional operator by angular max pooling defined for any function $h : X \times S^1 \rightarrow \RR$ by:
\[
\mathrm{amp}(h)(x) := \sup \{ |h(x, \theta)|, \ \theta \in S^1 \}
\]
This method however has a major drawback compared to usual convolutional neural networks on euclidean domains (e.g. images). Due to the angular max pooling the directional relationship between the filters of two convolutional layers is lost. We propose to remedy to this limitation by synchronizing the convolutional layers by transporting the frames used to compute the second layer to the rest of the surface using parallel transport so that the choice of frame used to compute the output the second layer induces choices of frames for the previous layer so that we know the relationship between the frames used to compute consecutive layers. To motivate our construction further we may come back to our interpretation of convolution over $\RR^n$:
\[
f * k ( x )
=
\langle \mathrm{Id}_x^*f,  \tau_{-x}^*k \rangle_{L^2(T_x \RR^n)}
\]
As we saw the exponential map can be seen as a generalization of $\mathrm{Id}_x$, we propose to also generalize $\tau_{-x}$. We have the following identification: $T_0 \RR^n = \RR^n$, therefore we can see $\tau_{-x}: T_x \RR^n \rightarrow T_0 \RR^n$ as a linear isometry. Note that $\tau_{-x}$ is the inverse of parallel transport operator along the geodesic joining $0$ to $x$. The choice of origin in $\RR^n$ and of orthonormal frame at the origin is arbitrary but whatever choice we do we can always transport the frame to all other points. We generalize this observation by introducing the notion of frame transporter, Let $X$ be a Riemannian manifold, for all $x \in X$ and $v \in T_x X$ denote by 
\[
\rho_{(x,v)}^X: T_x X \rightarrow T_{\exp^X_x(v)}
\]
the parallel transport operator along the geodesic path $t \in [0, 1] \mapsto \exp_x^X(tv)$ starting at $x$ with speed $v$. The map $\rho_{(x,v)}^X$ being a linear isometry it sends frames over $x$ to frames over $\exp^X_x(v)$.
\begin{Definition}[Frame transporter]
Let $X$ be a Riemannian manifold and
\[
TX \times_X FX := \bigsqcup_{x \in X} T_x X \times F_x X
\]
The frame transporter of $X$ is the map:
\[
\begin{array}{l|rcl}
F^X : & TX \times_X FX & \longrightarrow & FX \\
    & (v, e) \in T_x X \times F_x X & \longmapsto & \rho_{(x,v)}^X(e)
\end{array}
\]
\end{Definition}
We define the convolution of a function $\tilde{f}: TX \times_X FX \rightarrow \RR$ by a template $k: \RR^n \rightarrow \RR$ by:
\[
\begin{array}{l|rcl}
\tilde{f} * k : & FX & \longrightarrow & \RR \\
    & e \in F_x X & \longmapsto & \int_{T_x X} \tilde{f}\vert_{T_x X \times F_x X}(\bullet, e) \ e^*k \ d\mu_x^X.
\end{array}
\]
We can now define the notion of synchronized convolution: 
\begin{Definition}
Let $f: FX \rightarrow \RR$ a function. We define its "synchronized" convolution by a function $k: \RR^n \rightarrow \RR$ by:
\[
f \star k := \big( (F^X)^*f \big) * k : FX \rightarrow \RR
\]
\end{Definition}
We have a projection map $\pi_{FX}: FX \rightarrow X$ sending $F_x X$ to $\{x\}$ therefore we can extend the notion of synchronized convolution to functions $f: X \rightarrow \RR$ by setting:
\[
f \star k := (\pi_{FX}^*f) \star k.
\]
We observe that this construction generalizes the usual notion of convolution in the following way: Let $f: \RR^n \rightarrow \RR$ we have:
\[
f \star k( e_x ) = f * k ( x )
\]
where $e_x$ is the transport of the canonical basis of $\RR^n$ to $T_x \RR^n$ and $f * k$ is the usual convolution. Notice that with this definition of convolution the convolution of a function over the frame bundle is still a function over the frame bundle. Following the definition of original patch operator proposed by \cite{MasBosBroVan15} We define the synchronized patch operator as follows:
\begin{Definition}[Synchronized patch operator]
Let $K: (\RR^n)^2 \rightarrow \RR_+$ a kernel the synchronized patch operator associated with $K$ is the map $\mathrm{SP}[K]$ sending any function $f: FX \rightarrow \RR$ to the function:
\[
\begin{array}{l|rcl}
f \star K : & (X \times \RR^n) \times_X FX & \longrightarrow & \RR \\
    & (y, e) \in \RR^n \times F_x X & \longmapsto & \frac{f \star K(y, \bullet)( e ) }{1 \star K(y, \bullet)( e )}
\end{array}
\]
\end{Definition}
For the associated synchronized geodesic convolutional layer on surfaces we propose a slightly different definition that \cite{MasBosBroVan15}. First, we no longer assume that the surface is oriented an second we take into account the distortion induced by passing to polar coordinates when evaluating the layer at a weight function $a: S^1 \times \RR_+$. Recall that the orthogonal group $\mathrm{O}(2)$ is composed of two connected components $\mathrm{O}_+(2) := \mathrm{SO}(2)$ and $\mathrm{O}_-(2)$ that are both isomorphic to the unit circle $S^1$. Denote by $\tau$ the complex conjugation and identify $e^{i\theta}$ with the rotation matrix of angle $\theta$. We have:
\[
\left\{
\begin{array}{l}
  \mathrm{O}_+(2) = \{e^{i\theta} \ \vert \ \theta \in [0, 2\pi] \} \} \\
  \mathrm{O}_-(2) = \{e^{i\theta}\tau \ \vert \ \theta \in [0, 2\pi] \} \} 
\end{array}
\right.
\]






\begin{Definition}[Synchronized geodesic convolutional layer (SGCL)]
Fix an arbitrary choice of frames $e_x$ over all $x \in X$. The synchronized geodesic convolutional layer associated to a kernel $K$ satisfying the symmetry condition $(*)$ is defined for any function $f: FX \rightarrow \RR$ and weight function $a: S^1 \times \RR_+ \rightarrow \RR$ by:
\[
\begin{aligned}
&
\mathrm{sgc}^X_K(a,f)(e^{i\theta}e_x) 
:=
\int_{\RR_+} \int_{S^1} a(t-\theta,r)f \star K(re^{it}, e_x) \ dt dr
\\
&
\mathrm{sgc}^X_K(a,f)(e^{i\theta}\tau e_x) 
:=
\int_{\RR_+} \int_{S^1} a(t-\theta,r)f \star K(re^{-it}, \tau e_x) \ dt dr
\end{aligned}
\]
\end{Definition}
Note that the choice of local frames $e_x$ defining the SGCL is arbitrary therefore we must study the impact of rotations and reflexions of the frames on the definition. We define the orthogonal group of $TX$ as the free product of the orthogonal groups of the tangent spaces over all points of $X$:
\[
\mathrm{O}(TX) := \prod_{x \in X} \mathrm{O}(T_x X)
\]
The group $\mathrm{O}(TX)$ acts transitively on $FX$ by:
\[
(\theta_x)_{x \in X}.(e_x)_{x \in X} 
:=
(\theta_x(e_x))_{x \in X}
\]
This action also extends to the space of function over $FX$ by:
\[
\theta.f( e ) 
:=
f( \theta^{-1}.e ).
\]
Suppose we are given two choices of frames $(e_x)_{x \in X}$ and $(u_x)_{x \in X}$ then there exists a unique $\theta \in \mathrm{O}(TX)$ such that:
\[
u_x := \theta_x^{-1} e_x, \ \forall x \in X.
\]
We have 


We say that an operator $\rho$ sending functions over $FX$ to function over $FX$ is rotation equivariant if:
\[
\rho( \theta.f ) = \theta.\rho( f ), \ 
\forall f: FX \rightarrow \RR, \ \forall \theta \in \mathrm{O}(FX).
\]
\begin{Proposition}[Equivariance of SGCL]
For any $a: S^1 \times \RR_+ \rightarrow \RR$ the operator $\mathrm{sgc}_K^X(a, \bullet)$ is rotation equivariant and 
\end{Proposition}
\begin{proof}

\end{proof}
The definition of SGCL can be extended to handle multiple channels. Let $k \in \NN^*$, denote by 
\[
F^k X
:=
\bigsqcup_{x \in X} (F_x X)^k.
\]
for each $i \in [|1,k|]$ denote by $F^{k,i} X \simeq FX$ the $i$-th component of $F^k X$. Let $f = (f_1, \dots, f_p): F^p X \rightarrow \RR$, a matrix $a \in M_{q,p}(L^2(S^1 \times \RR_+, \RR))$ and a collection of frames $(e^1_x, \dots, e^q_x) \in (F_X X)^q$ we define the multi channel SGCL $\mathrm{sgc}^X_{K,p,q}(a, f): F^q X \rightarrow \RR$ by:
\[
\mathrm{sgc}^X_{K,p,q}(a, f)(e_x^i) 
:=
\sum_{j = 1}^p \mathrm{sgc}_K^X(a_{ij}, f_j)(e_x^i).
\]
The action of $\mathrm{O}(TX)$ extends to $F^k X$ and the space of function over $F^k X$ by acting on each of the factors $F^{k,i} X$. A parametric operator $\rho_{\theta \in \Theta}$ is a family of operators indexed by a parameter space $\Theta$. We denote by $\mathrm{Op}^X(p, q, \Theta)$ the space of parametric rotationally equivariant operators on $X$ with parameter space $\Theta$ sending functions over $F^pX$ to function over $F^qX$.
The equivariance still holds in the multichannel setting, that is for any subset $V \subset M_{q,p}(L^2(S^1 \times \RR_+, \RR))$ :
\[
\mathrm{sgc}^X_{K,p,q}(a, \bullet)_{a \in V}
\in
\mathrm{Op}^X(p, q, V)
\]


\begin{Definition}[SGCNN]
A rotationally synchronized neural network is the data of a sequence of integers $q_1, \dots, q_n$ and a sequence of parametric operators 
\end{Definition}

Note that the choice of frames $e_x$ used to define the synchronized geodesic convolutional layer is arbitrary however. The following proposition is a key component of our contribution it shows that this ambiguity is consistent across layers in construction of synchronized geodesic convolutional neural network is equivariant under the action of the orthogonal group on frames, 

\begin{Proposition}

\end{Proposition}

\subsection{synchronized covolution}

define the synchronized convolution

\subsection{synchronized patch operators}

define the synchronized and composite synchronized patch operators and their discretization.

\subsection{synchronized GCNN}


\section{Discretization over triangle meshes}
